On Optimality Conditions in Control Theory

We study optimality conditions for various types of control problems like the standard optimal control problem, optimal multiprocesses, problems with infinite horizon or the control of Volterra integral equations. To derive necessary conditions the needle variation method of Ioffe & Tichomirov is the central tool. In the particular control problem with infinite horizon the question of a suitable setting arises. We propose the framework of continuous state trajectories converging at infinity. This requires a version of Riesz' representation theorem and the introduction of regular Borel measures on the extended real number line. The control of Volterra integral equations including an inner and outer time variable. Consequently, we deal with a two-dimensional time set. We extend the needle variation method of Ioffe & Tichomirov to this case. The obtained optimality conditions are demonstrated in illustrative examples.

==> Symbole.tex <==
\section*{Liste der wichtigsten Symbole}
\begin{tabular}{lcl}
$\R$ &--& reelle Zahlengerade $(-\infty,\infty)$ \\[1mm]
$\R_+$ &--& unendlicher Zeithorizont $[0,\infty)$ \\[1mm]
$\overline{\R}_+$ &--& Abschluss $[0,\infty]$ von $\R_+$ \\[1mm]
$H$ &--& Pontrjagin-Funktion \\[1mm]
$\mathscr{H}$ &--& Hamilton-Funktion \\[1mm]
$\mathscr{L}$ &--& Lagrange-Funktion \\[1mm]
$C_b(I,\R^n)$ &--& Raum der beschr"ankten stetigen Funktionen, S.\,\pageref{Cb} \\[1mm]
$C(I,\R^n)$ &--& Raum der stetigen Funktionen, S.\,\pageref{C} \\[1mm]
$C_0(\R_+,\R^n)$ &--& Raum der stetigen Funktionen, die im Unendlichen \\
                 &  & verschwinden, S.\,\pageref{C0} \\[1mm]
$C_{\lim}(\R_+,\R^n)$ &--& Raum der stetigen Funktionen, die im Unendlichen einen \\
                      &  & Grenzwert besitzen, S.\,\pageref{Clim} \\[1mm]
$C_1(I,\R^n)$ &--& Raum der stetig differenzierbaren Funktionen, S.\,\pageref{C1} \\[1mm]
$L_p(I,\R^n)$ &--& Lebesgue-Raum, S.\,\pageref{Lp} \\[1mm]
$W^1_p(I,\R^n)$ &--& Sobolev-Raum, S.\,\pageref{W1p} \\[1mm]
%$W^1_{p,\lim}(\R_+,\R^n)$ &--& Sobolev-Raum der absolutstetigen Funktionen, die im Unend- \\
%                      &  & lichen einen Grenzwert besitzen, S.\,\pageref{W1plim} \\[1mm]
%$\ell_p$ &--& Folgenr"aume, S.\,\pageref{Ellp} \\[1mm]
%$\ell_{p,\lim}$ &--& R"aume konvergenter Folgen, S.\,\pageref{Ellplim} \\[1mm]
$\|\cdot\|$ &--& Euklidische Norm \\[1mm]
$\|\cdot\|_\infty$ &--& Supremumsnorm \\[1mm]
$\|\cdot\|_{L_p}$ &--& $L_p-$Norm \\[1mm]
$\|\cdot\|_{W^1_p}$ &--& $W^1_p-$Norm \\[1mm]
%$\|\cdot\|_{W^1_{p,\lim}}$ &--& $W^1_{p,\lim}-$Norm \pageref{W1plimNorm} \\[1mm]
${\rm conv\,} M$ &--& konvexe H"ulle der Menge $M$ \\[1mm]
$f'(x;z)$ &--& Richtungsableitung, S.\,\pageref{Richtungsableitung} \\[1mm]
$f^\circ(x;z)$ &--& Clarkescher Gradient, S.\,\pageref{ClarkescherGradient} \\[1mm]
$\partial f(x)$ &--& Subdifferential der Funktion $f$, S.\,\pageref{Subdifferential} \\[1mm]
$\partial_x f(x,y)$ &--& Subdifferential der Abbildung $x \to f(x,y)$, S.\,\pageref{partSubdifferential}
\end{tabular}
